Semantic Layout Manipulation with High-Resolution Sparse Attention

We tackle the problem of semantic image layout manipulation, which aims to manipulate an input image by editing its semantic label map. A core problem of this task is how to transfer visual details from the input images to the new semantic layout while making the resulting image visually realistic. Recent work on learning cross-domain correspondence has shown promising results for global layout transfer with dense attention-based warping. However, this method tends to lose texture details due to the resolution limitation and the lack of smoothness constraint of correspondence. To adapt this paradigm for the layout manipulation task, we propose a high-resolution sparse attention module that effectively transfers visual details to new layouts at a resolution up to 512x512. To further improve visual quality, we introduce a novel generator architecture consisting of a semantic encoder and a two-stage decoder for coarse-to-fine synthesis. Experiments on the ADE20k and Places365 datasets demonstrate that our proposed approach achieves substantial improvements over the existing inpainting and layout manipulation methods.

==> sections/conclude.tex <==
\section{Conclusion and Future Work}
\vspace{-0.05in}
In this paper, we investigate a challenging semantic layout manipulation task and present a high-resolution sparse attention module that can transfer high-resolution visual details from input images. We leverage our proposed key index sampling step and sparse attentive warping step to enable efficient computation. Based on the trained attention module, we also present a semantic guided generator architecture consisting of a semantic encoder and a two-stage decoder for coarse-to-fine synthesis. We perform extensive experiments on the ADE20k and Places2 datasets to validate the effectiveness of our method on both semantic-guided inpainting and semantic layout manipulation.
Our current approach applies warping at the highest-resolution, thus a multi-scale design would benefit the generated warping. Moreover, the current key index sampling procedure is non-differentiable. Better sampling strategies should be investigated to facilitate better sparse attention computation.
%In the future, we plan to explore multi-scale design and differentiable key index sampling to improve the performance and efficiency of our approach.

%\cl{Perhaps we should mention the limitation of our approach somewhere? Can be in conclusion?} \hz{added future work.} \cl{"better" is very vague. Also, future work does not equal limitation of current approach}
%\hz{revised.}

%\zl{for future work, I would very briefly suggest a potential future research direction, instead of listing many possible incremental improvements. Keep the future work part brief. For example, you could mention that current method does not work perfectly on manipulating layouts of structured objects, and a potential future research direction is to extend our model to improve semantic object manipulation.}
% To make the high-resolution attention feasible
% To propagate information between structurally uncorrelated and semantically unaligned scenes, we propose an MSCA module that leverages decoupled cross-attention for adaptive correspondence modeling. With MSCA, we propose a unified model for joint global-local alignment and image synthesis. We further propose a patch-based self-supervision scheme that enables training. Experiments on the COCO-stuff dataset show significant improvements over the existing methods. Furthermore, our approach provides interpretability and can be extended to other content manipulation tasks.

% We propose to address a challenging example-guided scene image synthesis task. To propagate information between structurally uncorrelated and semantically unaligned scenes, we propose an MSCA module that leverages decoupled cross-attention for adaptive correspondence modeling. With MSCA, we propose a unified model for joint global-local alignment and image synthesis. We further propose a patch-based self-supervision scheme that enables training. Experiments on the COCO-stuff dataset show significant improvements over the existing methods. Furthermore, our approach provides interpretability and can be extended to other content manipulation tasks.

==> sections/experiment.tex <==
\vspace{-0.3in}
\section{Experiments}
\label{sec:experiment}
\subsection{Implementation Details}
\label{sec:experiment_implementation}
% \noindent \textbf{Implementation Details} \quad
We train our high-resolution sparse attention model on the ADE20k dataset~\cite{ade20k} for 60 epochs.
% We apply the correspondence distillation loss in the first 20 epochs and remove the loss for the rest of the training.
Then we train semantic layout manipulation model on the Places365~\cite{places2} dataset.
We generate semantic label maps on Places365 using the HRNets~\cite{hrnet} model pretrained on ADE20k dataset. During testing, we apply a refinement network~\cite{cascadepsp} to post-process the predicted labels maps. More training details are provided in the Appendix.
% The first and the second stage models are trained with batch sizes of 64 and 16, respectively. We use Adam~\cite{adam} as the optimizer with a learning rate of 0.0002 to train both models. During testing, we apply a segmentation refinement network~\cite{cascadepsp} to post-process the predicted semantic labels.

\subsection{Comparisons with Existing Methods}
\label{sec:experiment_compare}
% \noindent \textbf{Comparison with State-of-the-arts methods} \quad
We compare our method with the state-of-the-art inpainting methods including  Deepfill-v2~\cite{deepfillv2}, Profill~\cite{profill}, Edge-connect~\cite{edgeconnect}, MEDFE~\cite{liu2020rethinking}, PatchMatch~\cite{patchmatch}, semantic layout manipulation methods including SESAME~\cite{sesame} and global layout editing method CoCosNet~\cite{cocosnet} on the ADE20k and Places365 validation sets. For those methods, we feed label maps (or edge map of the label maps) whenever possible. 

\zht{
\noindent \textbf{Quantitative Evaluation} \quad
We use \textit{reconstruction} and \textit{manipulation} tasks to evaluate our method. The reconstruction task is adapted from the guided inpainting~\cite{deepfillv2,sesame} to reconstruct groundtruth images from masked images and guided inputs (such as label maps or edge maps).
The manipulation task aims to generate a manipulated image using a locally edited label map. To generate such an evaluation set, we randomly sample a segment from the evaluation images and apply random affine transformation on the segment to generate the image before editing. Fig.~\ref{fig:main_compare} shows the resulting synthetic data. For fair comparisons on the reconstruction task, we modify our warping stage 
% Unlike the inpainting baselines, our method is designed to warp pixels inside the mask for better image manipulation.
such that the attention weights for the masked region are set to 0 and pixels inside the mask are ignored in the attention-based alignment stage.
% The input format detail are shown in Table~\ref{tab:input}. 
}

\begin{table}[]
	\caption{Quantitative evaluation on the reconstruction and manipulation tasks. Higher scores are better for the metrics with uparrow ($\uparrow$), and vice versa. 
	}
	\centering
	\resizebox{\columnwidth}{!}{
	\begin{tabular}{ |l|c|c|c|c|c|c|}
    %   \toprule
    %   \toprule
		\hline
		\hline
		Methods                             &$\ell_1$ err. $\downarrow$ &	PSNR$\uparrow$ & SSIM$\uparrow$ &  LPIPS$\downarrow$	& FID$\downarrow$ & $\mathcal{L}_{\text{style}}$~\cite{gatys2015neural}$\downarrow$\\
		\hline
		\multicolumn{7}{|l|}{\em ADE20k reconstruction}\\
		\hline
		Deepfill\_v2~\cite{deepfillv2}&  0.02959&  21.762&  0.844 & 0.305& 85.73 &4.440e-06\\
		MEDFE~\cite{liu2020rethinking}&  0.03825&  20.730&  0.808& 0.413& 167.12 &1.528e-05\\
		Profill~\cite{profill}&  0.02875&  22.405&  0.848& 0.317& 97.78&8.183e-06\\
		Edge-connect~\cite{edgeconnect}&  0.04512&  20.179&  0.742 & 0.284& 80.96&6.061e-06\\
		SESAME~\cite{sesame}&  0.06032&  18.505&  0.720 & 0.319& 66.45&1.300e-05\\
% 		CoCosNet~\cite{cocosnet}&  0.03600&  20.678&  0.823 & 0.317& 99.68&6.281e-06\\
% 		Ours&  \best{0.02384}&  \best{23.048}&  \best{0.870} & \best{0.249}& \best{58.27}&\best{2.78e-06}\\
		Ours&  \best{0.02486}&  \best{23.173}&  \best{0.863} & \best{0.217}& \best{49.42}&\best{2.800e-06}\\
		\hline
		\multicolumn{7}{|l|}{\em ADE20k manipulation}\\
		\hline
% 		deepfill\_v2~\cite{deepfillv2}&  0.02959&  21.762&  0.844 & 0.305& 85.73 &4.40e-06\\
% 		MEDFE~\cite{liu2020rethinking}&  0.03825&  20.730&  0.808& 0.413& 167.12 &1.53e-05\\
% 		profill~\cite{profill}&  0.02875&  22.405&  0.848& 0.317& 97.78&8.35e-06\\
		SESAME~\cite{sesame}&  0.03561&  20.825&  0.834 & 0.178& 47.40& 5.281e-06\\
		CoCosNet~\cite{cocosnet}&  0.03065&  24.063&  0.837 & 0.165& 98.13&\best{1.397e-06}\\
% 		Ours&  \best{0.02968}&  \best{22.255}&  \best{0.856} & \best{0.139}& \best{29.15}&\best{2.729e-06}\\
		Ours&  \best{0.02827}&  \best{22.672}&  \best{0.859} & \best{0.136}& \best{28.07}&2.597e-06\\
		\hline
		\multicolumn{7}{|l|}{\em Places365 reconstruction}\\
		\hline
		Deepfill\_v2~\cite{deepfillv2}&  0.06012&  18.145&  0.688 & 0.297& 104.00 &\best{4.082e-06}\\
		MEDFE~\cite{liu2020rethinking}& 0.07053&  17.498&  0.652& 0.402& 160.86 &3.672e-05\\
		Profill~\cite{profill}& 0.05597&  18.758&  0.699 & 0.298& 103.17&1.211e-05\\
		Edge-connect~\cite{edgeconnect}&  0.05448&  19.158&  0.694 & 0.286& 97.21&6.517e-06\\
		SESAME~\cite{sesame}&  0.06050&  18.586&  0.684 & 0.326& 119.72&1.406e-05\\
		CoCosNet~\cite{cocosnet}&  0.07759&  16.841&  0.644 & 0.356& 134.80&1.235e-05\\
% 		CoCosNet**~\cite{cocosnet}&  0.02948&  24.296&  0.842 & 0.254& 63.77&3.064e-06\\
% 		Ours&   \best{0.05419}&  \best{19.177}&  \best{0.708} & \best{0.268}& \best{89.25} &\best{2.719e-06}\\
		Ours&   \best{0.05209}&  \best{19.478}&  \best{0.714} & \best{0.254}& \best{84.68} &5.811e-06\\
		\hline
		\multicolumn{7}{|l|}{\em Places365 manipulation}\\
		\hline
% 		Deepfill\_v2\_edge~\cite{deepfillv2}&  0.06012&  18.145&  0.688 & 0.297& 104.00 &4.082e-06\\
		SESAME~\cite{sesame}&  0.02617&  22.957&  0.879 & 0.118& 49.24&1.831e-06\\
		CoCosNet~\cite{cocosnet}&  0.03050&  22.979&  0.873 & 0.126& 47.47&1.397e-06\\
% 		CoCosNet**~\cite{cocosnet}&  0.02521&  24.432&  0.890 & 0.114& 41.271&5.501e-07\\
% 		CoCosNet***~\cite{cocosnet}&  0.02566&  24.373&  0.888 & 0.112& 40.57&5.646e-07\\
% 		Ours&  \best{0.02796}&  \best{23.002}&  \best{0.880} & \best{0.106}& \best{33.83} &\best{1.107e-06}\\
		Ours &  \best{0.02500}&  \best{24.252}&  \best{0.888}& \best{0.102} & \best{31.35}& \best{6.801e-07}\\
		\hline
		\hline
	\end{tabular}
	}
	\label{tab:main_experiment_reconstruct}
\end{table}


% \begin{table}[]
%     \caption{Quantitative evaluation on the manipulation task.
%     % 	in terms of $\ell_1$ error, PSNR, SSIM~\cite{ssim}, LPIPS\cite{lpips}, Fréchet Inception Distance (FID)~\cite{fid} and the style loss from~\cite{gatys2015neural} .
%     Higher scores are better for the metrics with uparrow ($\uparrow$), and vice versa.
% 	}
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% 	\begin{tabular}{ |l|c|c|c|c|c|c|}
%     %   \toprule
%     %   \toprule
% 		\hline
% 		\hline
% 		Methods                             &$\ell_1$ err. $\downarrow$ &	PSNR$\uparrow$ & SSIM$\uparrow$ &  LPIPS$\downarrow$	& FID$\downarrow$ & $\mathcal{L}_{style}$~\cite{gatys2015neural}$\downarrow$\\
% 		\hline
% % 		\multicolumn{7}{|l|}{\em ADE20k}\\
% % 		\hline
% % % 		deepfill\_v2~\cite{deepfillv2}&  0.02959&  21.762&  0.844 & 0.305& 85.73 &4.40e-06\\
% % % 		MEDFE~\cite{liu2020rethinking}&  0.03825&  20.730&  0.808& 0.413& 167.12 &1.53e-05\\
% % % 		profill~\cite{profill}&  0.02875&  22.405&  0.848& 0.317& 97.78&8.35e-06\\
% % 		SESAME~\cite{sesame}&  0.03561&  20.825&  0.834 & 0.178& 47.40& 5.281e-06\\
% % 		CoCosNet~\cite{cocosnet}&  0.03454&  21.505&  0.843 & 0.165& 40.76&3.144e-06\\
% % % 		Ours&  \best{0.02968}&  \best{22.255}&  \best{0.856} & \best{0.139}& \best{29.15}&\best{2.729e-06}\\
% % 		Ours&  \best{0.02827}&  \best{22.672}&  \best{0.859} & \best{0.136}& \best{28.07}&\best{2.597e-06}\\
% % 		\hline
% % 		\multicolumn{7}{|l|}{\em Places365}\\
% % 		\hline
% % % 		Deepfill\_v2\_edge~\cite{deepfillv2}&  0.06012&  18.145&  0.688 & 0.297& 104.00 &4.082e-06\\
% % 		SESAME~\cite{sesame}&  0.02617&  22.957&  0.879 & 0.118& 49.24&1.831e-06\\
% % 		CoCosNet~\cite{cocosnet}&  0.03176&  22.266&  0.868 & 0.127& 48.20&1.312e-06\\
% % % 		CoCosNet**~\cite{cocosnet}&  0.02521&  24.432&  0.890 & 0.114& 41.271&5.501e-07\\
% % % 		CoCosNet***~\cite{cocosnet}&  0.02566&  24.373&  0.888 & 0.112& 40.57&5.646e-07\\
% % % 		Ours&  \best{0.02796}&  \best{23.002}&  \best{0.880} & \best{0.106}& \best{33.83} &\best{1.107e-06}\\
% % 		Ours &  \best{0.02500}&  \best{24.252}&  \best{0.888}& \best{0.102} & \best{31.35}& \best{6.801e-07}\\
% % 		deepfill\_v2~\cite{deepfillv2}&  &  &   & &  &\\
% 		\hline
% 		\hline
% 	\end{tabular}
% 	}
% 	\label{tab:main_experiment_manipulate}
% \end{table}
\vspace{-0.2in}
For quantitative measurement, we apply average L1 Error ($\ell_1$), PSNR and SSIM~\cite{ssim} as the low-level metrics and Frchet Inception Distance (FID)~\cite{fid}, Perceptual Image Patch Similarity Distance (LPIPS)~\cite{lpips} and the style similarity loss $\mathcal{L}_{\text{style}}$ of~\cite{gatys2015neural} as perceptual-level metrics. Results on manipulation and reconstruction tasks are 
%shown 
in Table~\ref{tab:main_experiment_reconstruct}.
For both tasks, our method performs the best according to most metrics. Additionally, we observe that the semantic-guided approaches (SESAME~\cite{sesame}, CoCosNet~\cite{cocosnet} and ours) in general outperforms other inpainting approaches.

\noindent \textbf{Qualitative Evaluation} \quad
Fig.~\ref{fig:main_compare} presents visual comparisons on the image manipulation task where input images are manipulated in regions indicated by the red rectangles. 
SESAME~\cite{sesame} generates coherent colors but produces structural artifacts (e.g. the tower in the last row), as the masked pixel is not leveraged by warping.
CoCosNet~\cite{cocosnet} better transfers appearance via alignment. However, CoCosNet hallucinates wrong objects (tower in the last row) as warping is performed in lower resolution and may contain error.
Moreover, CoCosNet often generates pixels that have incoherent colors with their surrounding due to the lack of local refinement step. In contrast, our method better preserves texture details of input images, generating more coherent results.

Fig.~\ref{fig:main_compare_inpaint} shows comparison from the reconstruction task.
%, where our approach is compared against inpainting approaches including Deepfill\_v2~\cite{deepfillv2}, MEDFE~\cite{liu2020rethinking}, Profill~\cite{profill} and semantic layout manipulation approaches including SESAME~\cite{sesame}, CoCosNet~\cite{cocosnet}. 
Benefiting from the semantic layout guidance, SESAME~\cite{sesame}, CoCosNet~\cite{cocosnet} and our approach better reconstructs image layout. Among them, our approach better preserves details from the inputs (e.g. texture of bed sheet, building). In addition, Fig.~\ref{fig:main_compare_handcraft} compares the image manipulation results on real data, where our method achieves the best visual results.

\zht{
Fig.~\ref{fig:corr_visualize} shows an example visualization of the correspondences generated by the proposed sparse attention module.
% Query positions in the edited image/layout, and their corresponding sparse key sets are shown via dots with the same color in the left and right figures, respectively.
Using the proposed selective sampling procedure, our sparse attention module can effectively locate regions of interest to enable efficient attention computation.
}

\begin{figure}[]
	\centering
	\includegraphics[width=0.9\linewidth]{sections/figures/corr_visualize.jpg}
	\caption{Correspondence generated by our sparse attention module. The colored points in the left and right figures represent the query position and the sampled sparse keys, respectively.}
% 	are represented by dot with the same color.
% 	For each query position (colored points on the left), our sparse attention module generates a sparse key index set (left) to accelerate attention computation.}
	\label{fig:corr_visualize}
\end{figure}


% We also conduct a user study and show the result in Table~\ref{tab:ablation}.  Specifically, we randomly select 25 images from the Place365 validation set for manipulation and reconstruction, respectively. We show results of each image to 9 users and ask them to select the best results. Finally, we collect 225 votes from all users for each dataset. Results in the table show that our method receives the majority of the votes on both manipulation and reconstruction tasks.


\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{sections/figures/main_compare.pdf}
	\caption{Qualitative comparisons on the manipulation task. We show from left to right the input image, target layout, and the results of SESAME~\cite{sesame}, CoCosNet~\cite{cocosnet} and our model, respectively. Best viewed by zoom-in.
% 	\zl{I would put ours in the last column.} \hz{done}
	}
	\label{fig:main_compare}
\end{figure}

\begin{figure}[]
	\centering
	\includegraphics[width=1\linewidth]{sections/figures/teaser-compare.jpg}
	\caption{Qualitative comparisons on the real manipulation task. Best viewed by zoom-in.}
	\label{fig:main_compare_handcraft}
\end{figure}

\begin{figure*}[t]
	\centering
	\includegraphics[width=1\linewidth]{sections/figures/main_compare_inpaint.pdf}
	\caption{Qualitative comparisons on the reconstruction task. We show from left to right the input image, target layout, and the results of Deepfill\_v2~\cite{deepfillv2}, MEDFE~\cite{liu2020rethinking}, Profill~\cite{profill}, SESAME~\cite{sesame}, CoCosNet~\cite{cocosnet} and our model, respectively. Best viewed by zoom-in.}
	\label{fig:main_compare_inpaint}
\end{figure*}

\vspace{-0.1in}
\subsection{Ablation Study}
We perform a set of ablation experiments to show the importance of the network design and usage of the high-resolution correspondence. Results of the ablations are shown in Table~\ref{tab:ablation}. To study the network design, we train four variants of our model: i) \textit{our w/o SE} that removes the \textbf{s}emantic \textbf{e}ncoder branch from the generator, ii) \textit{our w/o CA} that removes the \textbf{c}ontextual \textbf{a}ttention branch from the two-stage encoder, iii) \textit{our w/o dilate} that removes the dilated convolution branch branch from the two-stage encoder, iv) \textit{our w/o IF} that does not feed the \textbf{i}ntermediate \textbf{f}eatures from coarse-stage decoder to the refinement network. From the result, our full model achieves the best performance on metrics that reflect structure-level similarity (SSIM) and semantic similarity (LPIPS, FID). We also observe that removing the contextual attention or dilated convolution branch impact performances the most suggesting that contextual propagation is important for local editing.
% \cl{What happens if you only use contextual attention but not dilated conv encoder in the two branch encoder?} \hz{done}
%\cl{The notations in the text does not match the notations in Table3}

To study the effect of the high-resolution correspondence, we adopt two variants of locally warped image $x_{\text{warp}}$ from Eq.~\ref{eq:local_align} to train models: i) \textit{our w/o corres} set $r_{x_0\rightarrow c_1}$ to $0$, resulting in a model that does not relies on correspondence, ii) \textit{our w/ LR corres} set $r_{x_0\rightarrow c_1}$ to the low-resolution warped image of CoCosNet~\cite{cocosnet}. From the results, we observe that the quality of correspondence impact the final performance. Benefiting from the high-resolution correspondence, our full model achieves the best performance while \textit{our w/ LR corres} achieves better performance than \textit{our w/o corres} due to the usage of correspondence. Notably, sharing similar input as SESAME~\cite{sesame}, \textit{our w/o corres} substantially outperforms SESAME~\cite{sesame}. More visual comparison is provided in the Appendix.
% \cl{Do we not have figure to show the results from the ablation study?}\hz{added description}

% Table~\ref{tab:ablation} shows the quantitative evaluation of those ablation models on the Places365 manipulation task.
% From the table, feeding the warped image to the two-stage generator substantially improves the model performance while the semantic encoder can further improve performance. Note that the improvements using the dedicated semantic encoder are reflected more on semantic-aware metrics such as LPIPS, FID, which are aligned better with visual quality.
% \zl{add a short analysis based on the final ablation results.} \cl{Table 3 is incomplete.}


\begin{table}[]
	\caption{Quantitative evaluation of the ablation models on the Places365 manipulation task.
    % Higher scores are better for the metrics with uparrow ($\uparrow$), and vice versa.
	}
	\centering
	\resizebox{\columnwidth}{!}{
	\begin{tabular}{ |l|c|c|c|c|c|c|}
    %   \toprule
    %   \toprule
		\hline
		\hline
		Methods                             &$\ell_1$ err. $\downarrow$ &	PSNR$\uparrow$ & SSIM$\uparrow$ &  LPIPS$\downarrow$	& FID$\downarrow$ & $\mathcal{L}_{\text{style}}$~\cite{gatys2015neural}$\downarrow$\\
		\hline
% 		SESAME~[35]&  0.02617&  22.957&  0.879 & 0.118& 49.24&1.831e-06\\
% 		CoCosNet~[55]&  0.03176&  22.266&  0.868 & 0.127& 48.20&1.312e-06\\
% 		CoCosNet (place365)~[55]&  0.03340&  21.822&  0.864 & 0.136 & 51.03 & 2.528e-06\\
% 		\hline
		ours full &  \best{0.02500}&  \best{24.252}&  \best{0.888}& \best{0.102} & \best{31.35}& 6.801e-07\\
		\hline
		ours w/o SE&  0.02525&  23.940&  0.887& 0.104& 33.51& \best{4.875e-07}\\
		ours w/o CA&  0.02629&  23.879&  0.885&  0.104& 32.18& 7.896e-07\\
		ours w/o dilate&  0.02602&  24.036&  0.885&  0.105& 32.43& 7.760e-07\\
		ours w/o IF& 0.02534&  24.100&  0.887& 0.105 & 33.02& 6.731e-07\\
		\hline
		ours w/o corres&  0.02764&  22.999&  0.877&  0.112& 38.61& 1.032e-06\\
		ours w/ LR corres& 0.02619&  23.751&  0.885& 0.104 & 32.65& 8.252e-07\\
% 		\hline
% 		ours w/o GAN& 0.02506&  24.508&  0.889& 0.104 & 32.82& 8.811e-07\\
% 		ours w/o perc& 0.02675&  23.792&  0.884& 0.112 & 38.05& 1.118e-06\\
		\hline
		ours retrained**& 0.02648&  23.831&  0.885& 0.103 & 32.85& 6.353e-07\\
		\hline
		\hline
	\end{tabular}
	}
	\label{tab:ablation}
\end{table}
\vspace{-4pt}


% \vspace{-8pt}
% \begin{table}[ht]
%     \caption{Quantitative evaluation on the manipulation task.
%     % Higher scores are better for metrics with uparrow ($\uparrow$), and vice versa.
%     }
% 	\centering
% 	\resizebox{\columnwidth}{!}{
% 	\begin{tabular}{ |l|c|c|c|c|c|c|}
%     %   \toprule
%     %   \toprule
% 		\hline
% 		\hline
% 		Methods (on {\em Place365})   &$\ell_1$ err. $\downarrow$ &	PSNR$\uparrow$ & SSIM$\uparrow$ &  LPIPS$\downarrow$	& FID$\downarrow$ & $\mathcal{L}_{style}$[17]$\downarrow$\\
% 		\hline
% % 		\multicolumn{7}{|l|}{\em Place365}\\
% % 		\hline
% % 		\multicolumn{7}{|l|}{\em Places365}\\
% % 		\hline
% % 		Deepfill\_v2\_edge~\cite{deepfillv2}&  0.06012&  18.145&  0.688 & 0.297& 104.00 &4.082e-06\\
% 		SESAME~[35]&  0.02617&  22.957&  0.879 & 0.118& 49.24&1.831e-06\\
% 		CoCosNet~[55]&  0.03176&  22.266&  0.868 & 0.127& 48.20&1.312e-06\\
% 		CoCosNet (place365)~[55]&  0.03340&  21.822&  0.864 & 0.136 & 51.03 & 2.528e-06\\
% 		\hline
% 		ours full &  \best{0.02500}&  \best{24.252}&  \best{0.888}& \best{0.102} & \best{31.35}& \best{6.801e-07}\\
% 		ours w/o Enc&  0.02525&  23.940&  0.887& 0.104& 33.51& 4.875e-07\\
% 		ours w/o CA&  0.02629&  23.879&  0.885&  0.104& 32.18& 7.896e-07\\
% 		ours w/o IF& 0.02534&  24.100&  0.887& 0.105 & 33.02& 6.731e-07\\
% 		\hline
% 		\hline
% 	\end{tabular}
% 	}
% 	\label{tab:ablation}
% \end{table}


% \begin{table}[]
% 	\caption{User preference for the results of each method. 
% 	}
% 	\centering
% % 	\resizebox{\columnwidth}{!}{
% 	\begin{tabular}{ |l|c|}
%     %   \toprule
%     %   \toprule
% 		\hline
% 		\hline
% 		Methods                             & Preference Votes\\
% 		\hline
% 		\multicolumn{2}{|l|}{\em Manipulation}\\
% 		\hline
% 		SESAME~\cite{supp_sesame}&  13\\
% 		CoCosNet~\cite{supp_cocosnet}&  14\\
% 		Ours&  198\\
% 		\hline
% 		\multicolumn{2}{|l|}{\em Reconstruction}\\
% 		\hline
% 		Deepfill\_v2~\cite{supp_deepfillv2}& 33 \\
% 		MEDFE~\cite{supp_liu2020rethinking}& 0\\
% 		Profill~\cite{supp_profill}& 23\\
% 		SESAME~\cite{supp_sesame}&  2\\
% 		CoCosNet~\cite{supp_cocosnet}&  3\\
% 		Ours&   164\\
% 		\hline
% 		\hline
% 	\end{tabular}
% % 	}
% 	\label{tab:ablation}
% \end{table}

%\vspace{-0.03in}
\subsection{Reference-based Layout Manipulation}
\label{sec:application}
\vspace{-0.05in}
Our model is flexible and can also take additional reference images as input for advanced layout manipulation. Some sample results are as shown in Fig.~\ref{fig:application}. The results show that our method can seamlessly re-synthesize and compose contents from multiple image sources.
% \zht{To achieve this, we first warp contents from the input image to the edited layout. Next, the user specifies the semantic region to borrow from the reference image.  That region is then warped towards the target layout and overlaid on the previously-warped result. Finally, the combined warp is sent to the generator for final synthesis.}
The generation procedure of reference-based manipulation and more visual results can be found in the Appendix.
%\cl{The description is not clear about how the fusion is done. What do you mean "fuse them according to the target semantic layout"?} \hz{done}
%\cl{What do you mean "specified semantics"?} \hz{use "intersted semantics"}\cl{I modified the paragraph above based on my understanding. Please check whether it is correct.} \hz{that's correct, thanks!}

\begin{figure}[]
	\centering
	\includegraphics[width=1\linewidth]{sections/figures/application.jpg}
	\caption{Example results of our method taking additional reference images to synthesize images with new semantic layouts. It can also be applied to other multi-image editing tasks such as image compositing and object insertion.}
	\label{fig:application}
	\vspace{-0.2in}
\end{figure}

% \subsection{Discussion}



==> sections/intro.tex <==
% Figure, describe task , local editing by manipulating semanti clayout. Previous work Sesame, semantic pyrimid, MIT David, SPGNet. Related to guided inpainting, works XXX. Limitation, discard information inside the mask, also cannot dramtic change. 

% Semantic pyrimid, cannot do large deformation (no explicite warpin). 

% On the other hand, warping-based, global layout manipulatino cocosnet, attention warping to warp texture, can do dramitc layout ediitng, but, they handle global editing, low-resolution non-smooth attention, but global is promising because handle large deformation reuse original inforamtion

% 强调ｇｌｏｂａｌ多一点，correspondence -based promising，但是correspondence 缺点.

% Combine advantage of two networks, we propose a unified ediitng model. To this end, we propose a higher resoluition , cross modal correpsondence, efficient sparse attention to genrate HR wapring as approxi to help layout. Details: approxi + layout , two stage decoder

% contribution: high-res attention, new semantic layout framework the combine advantage guided inptainting and global layout warping, experiment STOA results.

% Figure, describe task , local editing by manipulating semanti clayout. popular with advance of GAN. 

\vspace{-0.1in}
\section{Introduction}

\label{sec:intro}
Semantic layout manipulation refers to the task of editing an image by modifying its semantic label map, i.e. changing the semantic layout or inserting/erasing objects as illustrated in Fig.~\ref{fig:teaser}. It has many practical image editing applications such as photo-editing~\cite{bau_semantic}, image retargeting~\cite{patchmatch}, restoration~\cite{sesame} and composition~\cite{SemanticPyramid}, but is relatively under-explored due to the challenges of predicting complex, non-rigid spatial deformations and the domain gap between the input image and the target semantic layout. Essentially, developing an effective method to transfer visual patterns from the input image to the target semantic layout is the key to solving the problem.

Early works~\cite{image_analogies,patchmatch,cho2008patch,Image_quilting} on image synthesis allow users to mark semantic regions for guided image manipulation. These methods utilize non-parametric modeling of patches~\cite{image_analogies,Image_quilting} or patch-based copy-pasting strategies~\cite{patchmatch,cho2008patch} to generate new images. They work well for generating stationary textures or repeating structures, but cannot hallucinate new semantic structures.
%nor generate new semantics in the resulting image. 

\begin{figure}[t]
	\centering
	\includegraphics[width=1.\linewidth]{sections/figures/teaser-teaser_LR.jpg}
	\caption{\textbf{Semantic layout manipulation.} Given an input image (1st column) and a semantic label map (3rd column) manipulated from an existing semantic map (2nd column), our network generates manipulated images (last column) that conform to the semantic layout guidance. The images are generated at resolution $512\times 512$.
% 	Note that our model is insensitive to noise from the noises of layout caused by semantic parser~\cite{hrnet}.
	It is worth noting that rather than relying on the ground-truth layout for manipulation, our model utilizes a semantic parser~\cite{hrnet} to generate layouts from input images.
% 	does not requires ground-truth layout. The original label map are generated using semantic parser~\cite{hrnet} and may contain noises.
	}
	\label{fig:teaser}
\end{figure}


Recently, with the development of deep generative models such as Generative Adversarial Networks (GANs), structure-guided image manipulation has made remarkable progresses. In particular, Champandard~\etal~\cite{champandard2016semantic} design a semantic-aware loss on a pretrained classifier~\cite{vgg} for semantic-guided artwork generation. Zhu~\etal~\cite{zhu2016generative} optimize the latent code of generative model for layout-constrained image generation.
More recently, guided inpainting methods~\cite{deepfillv2,spg,edgeconnect} are proposed to manipulate nature images. Specifically, guided inpainting approaches mask out some regions from images and hallucinate new pixels to encourage the inpainting results to follow the edge scribbles provided by users.  To achieve semantic layout manipulation, a recent work~\cite{sesame} extends inpainting networks by including semantic label maps in the missing region as inputs. Despite showing promising results,~\cite{sesame} is inherently limited in that (1) it discards pixels inside the mask region which may contain important visual details useful for manipulation tasks, (2) it lacks the spatial alignment mechanism to handle drastic layout change.   

On the other hand, methods utilizing attention-based warping~\cite{cocosnet,msca} have shown promising results for global reference-based layout editing.
% \todo{or example-guided synthesis}
Specifically, Zhang~\textit{et al.}~\cite{cocosnet} introduce a cross-domain correspondence network to warp input images to desired layouts.
Zheng~\textit{et al.}~\cite{msca} propose a spatial-channel attention method to align multi-scale visual features to a new layout.
Due to explicit warping, they can handle dramatic layout changes.
However, the global layout editing task does not take into account the contextual information from the input image and manipulation intention from users. Naively applying global warping for local manipulation 
tasks will also modify the surrounding image contents and is undesirable.
More critically, the warping schemes of~\cite{cocosnet,msca} are computationally costly, and thus are limited to low-resolution warping~\cite{cocosnet} or are applied to individual regions independently~\cite{msca}, causing the loss of visual details in the warped image.
% Nevertheless, global editing is promising for local manipulation task as it can handle large layout deformation while being able to reuse information from the mask region. \cl{What is the sentence above trying to convey? Arguing for the advantage of [23] and [26]?}
% Combining the advantage of inpainting-based approach and warping-based approach, we proposed a unified editing framework. T

Inspired by the above observations, we extend the guided image inpainting framework to also incorporate a warped version of the original image itself as an additional information source to help the local manipulation task. This strategy perfectly overcomes the limitations of both guided inpainting and global attention-based warping method for local manipulation tasks:  (1) guided inpainting framework allows it to exploit contextual information sufficiently for smooth generation, (2) attention warping schemes provide essential texture/structure information from the entire original image including editing regions. For the resolution limitation of attention-based warping, inspired by the PatchMatch~\cite{patchmatch} algorithm, we design a new algorithm to efficiently compute dense correspondences at high-resolution using sparse sampling of feature matches and iterative match propagation between the original image and edited layout. \zht{Compared to the existing work~\cite{cocosnet} that computes correspondence on the $4\times$ down-sampled images, our designed module can transfer visual details at the full resolution of input images.}%\zl{I thought we can do 512x512 while cocosnet can only handle 64x64}

% \hz{explain high-resolution attention , abstract, compare with existing work, compute attention on high-res feature map}
% \cl{We need higher level motivation and description of the key index sampling algorithm. As it stands right now in the introduction, it is not clear what it is about without reading the later sections of the paper.}
% \cl{We also need to talk about what are "the best of the both worlds" our unified framework is leveraging.}
\zht{
To this end, we first introduce a sparse attention module to efficiently warp high-resolution contents from an input image to a target layout. The attention module is based on two key components, namely 1) key index sampling and 2) sparse attentive warping to respectively generate and transfer visual details from a sparse set of features from the original image to each spatial location of the target layout. Next, we propose a unified semantic layout generator network to produce final manipulation results based on the masked original image, target layout, and the warped proxy output. The network is composed of a semantic encoder and a coarse-to-fine synthesis network and is trained based on a novel self-supervised training scheme. \zht{Recently, a concurrent work~\cite{zhou2020full} proposes a recurrent model to compute full-resolution correspondences. Different from~\cite{zhou2020full}, we aim to improve the efficiency of attention. Using our proposed sparse attention module, correspondence can be directly estimated on high-resolution feature maps.
Different from global layout transfer, local manipulation also requires new design and supervision to take into account contextual clues and the manipulation intention.
To address those challenges, we propose a new network architecture and a self-supervised scheme to tackle local editing.}%\zl{It might be good if we can briefly explain why local manipulation needs different design than global layout transfer.}\hz{revised}
%\cl{Does your explanation mean our sparse attention model is faster than the recurrent model[60]? Maybe should specifically call out the advantage of our approach rather than saying addressing a different problem?} \hz{Text is revised.}

% In particular, our attention module contains i) feature map up-sampling layers, ii) an efficient key index sampling algorithm that generates a set of matching key features (from the original image) for each query feature (from the target layout), and iii) a sparse attention warping module that attentively combines the sparse keys to generate high-resolution warped output.  
}

% \cl{I wonder whether we should call out in the introduction why do we need three stages? What benefit does contextual information bring us for local layout manipulation.}

Our main contributions are four-fold:
\begin{itemize}
    \vspace{-0.1in}
    \item An efficient sparse attention module to transfer visual details at a high $512\times512$ resolution. 
    \vspace{-0.1in}
    \item A unified semantic layout manipulation framework that takes advantages of both guided inpainting and global layout warping techniques. 
        \vspace{-0.1in}
    \item A novel self-supervised training scheme to train the semantic layout manipulation network.
        \vspace{-0.1in}
    \item Experiments on ADE20k and Places365 showing that our method achieves substantial improvements over the state-of-the-art inpainting and semantic layout manipulation methods.
\end{itemize}


% sample the sparse key
% We exploit spatial coherency of correspondence to generate 

% based on sparse attention to generate high-resolution warping. Our proposed warping module take advantage of the 






% \section{Introduction}
% \label{sec:intro}
% \begin{figure}[]
% 	\centering
% 	\includegraphics[width=0.88\linewidth]{sections/figures/teaser.pdf}
% % 	\includegraphics[width=1.0\linewidth]{sections/figures/exp_attention2.pdf}
% 	\caption{The inputs to style-consistent scene image generation is a  \emph{structurally uncorrelated} and \emph{semantically unaligned} segmentation map (column 1) and a reference image (column 2) that constraints the style of the output. The corresponding reference segmentation map is also taken as input. In spite of the complexity of the task, our model can generate high-quality scene images with a consistent style with the reference image.
% 	%\todo{change image, better result. add an arrow, so that it looks like 3:4}
%     }
% 	\label{fig:teaser}
% \end{figure}

% Conditional generative adversarial network (cGAN)~\cite{conditionalGAN} has recently made substantial progresses in realistic image synthesis. In cGAN, a generator $\hat{x}=\G(c)$ aims to output a realistic image $\hat{x}$ with a constraint implicitly encoded by $c$. Conversely, a discriminator $\D(x,c)$ learns such a constraint from ground-truth pairs $\langle x,c\rangle$ by predicting if $\langle \hat{x},c\rangle$ is real or generated. 

% The current cGAN models~\cite{spade,pix2pixhd,pix2pix} for semantic image synthesis aim to solve the \emph{structural consistency} constraint where 
% % \haofu{$c$ is a semantic label map and the output $x$ is required to structurally aligned with $c$.}
% % \haofu{The limitation of the direct semantic image synthesis is that the styles of the output images are inherently decided by the model and cannot controlled by users.} 
% % still uncontrollable to users, as users are agnostic about the style of outputs.
% the output image $x$ is required to be aligned to a semantic label map $c$.
% The limitation of the above generative process is that the styles of the image outputs are inherently determined by the model and thus cannot be controlled by users. To provide desired controllability over the generated styles, previous studies~\cite{example_cvpr18,example_cvpr19} 
% \haofu{impose additional constraints and allow more inputs to the generator:} $\hat{x}_{2 \rightarrow 1} =\G(z, c_1, x_2)$,
% % \zht{allow for an extra exemplar image to guides the output styles. Formally,}
% where $x_2$ is an exemplar image that guides the style of $c_1$. However, previous studies are designed on datasets such as face~\cite{liu2015deep,rossler2018faceforensics}, dancing~\cite{example_cvpr19} or street view~\cite{yu2018bdd100k}, where the input images usually contain similar semantics and the spatial structures of $y$ and $c_x$ are usually similar as well.

% \haofu{Different from the previous studies, we propose to address a more challenging example-guided \emph{scene image} generation task. As shown in Fig.~\ref{fig:teaser}, given a semantic label map $c_1$ (column 1) and an arbitrary scene image $x_2$ (column 2) with its semantic map $c_2$ (column 3) as the input, the task aims to generate a new scene image $\hat{x}_{2 \rightarrow 1}$ (column 4) that matches the semantic structure of $c_1$ and the scene style of $x_2$. The challenge is that scene images have complex semantic structures as well as diversified scene styles, and more importantly, the inputs $c_1$ and $x_2$ are \emph{structurally uncorrelated} and \emph{semantically unaligned}. Therefore, a mechanism is required to better match the structures and semantics for coherent outputs, e.g., the tree styles can be applied to mountains but cannot be applied to sky.}

% %\zht{Different from the previously studied tasks~\cite{example_cvpr18,example_cvpr19,example_iclr19}, we study a more challenging example-guided \emph{scene image} generation task. Our task takes an arbitrary scene image with its semantic label map (in Fig.~\ref{fig:teaser} column 2 and 3, respectively) as exemplar-guidance to synthesize a new scene image (in Fig.~\ref{fig:teaser} column 4). Ours inputs are both \emph{structurally uncorrelated} and \emph{semantically unaligned}. Hence, a better mechanism is required to propagate information.}

% % the reference images (column 3) contains high-quality visual at each semantic regions. However, the reference images are structurally unrelated to the given conditions (column 1) and contains multiple new semantic regions while missing others. As a result, a more sophisticated mechanism than feature concatenation is demanded to propagate information from the reference images.

% \haofu{In this paper, we propose a novel Masked Spatial-Channel Attention (MSCA) module (Section~\ref{subsect:spatialchannel}) to propagate features across unstructured scenes. Our module is inspired by a recent work~\cite{doubleattention} for attention-based object recognition, but we apply a new cross-attention approach to model the semantic correspondence for image synthesis instead. To facilitate example-guided synthesis, we further improve the module by including: i) feature masking for semantic outlier filtering, ii) multi-scaling for global and local feature processing, and iii) resolution extending for image synthesis. As a result, our module provides both clear physical meaning and interpretability for the example-guided synthesis task.}

% %\zht{In this paper, we propose novel Masked Spatial-Channel Attention (MSCA) module (Section~\ref{subsect:spatialchannel}) to propagate features across unstructured scenes. Our module is inspired by a recent work~\cite{doubleattention} for attention modeling. Differently, we apply cross-attention to model correspondence for image synthesis. Moreover, improvements are made in the following aspects: i) feature masking for semantic outlier filtering, ii) multi-scaling for better feature aggregation, and iii) the extended resolution for image synthesis. Finally, our module owns clear physical meaning and interpretability for the example-guided synthesis task.} 

% \haofu{We formulate the proposed approach under an unified synthesis network for joint feature extraction, alignment and image synthesis. We achieve this by applying MSCA modules to the extracted features for multi-scale feature domain alignment. Next, we apply a recent feature normalization technique, SPADE~\cite{spade} on the aligned features to allow spatially-controllable synthesis. To facilitate the learning of this network, we propose a novel patch-based self-supervision scheme. As opposed to~\cite{example_cvpr19}, our scheme requires only semantically parsed images for training and does not rely on video data.
% % for semantic matched pairs $c_1$ and $x_2$. 
% We show that a model trained with this approach generalizes over scales and across different scene semantics.
% }

% %\zht{Next, we propose an end-to-end synthesis network (Figure~\ref{fig:generator}) for joint feature extraction, alignment and image synthesis. We achieves this by applying MSCA modules on the extracted features for multi-scale feature domain alignment. We apply a recent feature normalization technique, SPADE~\cite{spade} on the aligned features to allow spatially-controllable synthesis.}

% %\zht{Finally, we propose a novel patch-based self-supervision scheme to enable training. Acquiring style-consistent pairs is known hard. Recent works on style-guided image-to-image translation~\cite{munit,lee2018diverse,example_iclr19} apply disentangle learning which separates style and content. However, it is less studied how to disentangle style and content from both semantic label maps and images. A more recent work~\cite{example_cvpr19} utilize videos to generate paired data. However, acquiring diversified scene videos can be hard. Instead, our self-supervision scheme requires only annotated images for training. We show that model trained with our data scheme generalizes over scales and across different scene semantics.}

% %\vspace{10pt}
% Our main contributions include the following:
%   \vspace{-0.08cm}
% \begin{itemize}
%     \item A novel masked spatial-channel attention (MSCA) module to propagate features for unstructured scenes. %Improvements over~\cite{doubleattention} are made including feature masking, multi-scaling and extended resolution.
%     \vspace{-0.08cm}
%     \item An unified synthesis network for joint feature extraction, alignment and image synthesis. %MSCA modules are applied for multi-scale feature domain alignment. A recent feature normalization techniques~\cite{spade} is used for spatially-controllable synthesis.
%     \vspace{-0.08cm}
%     \item A novel patch-based self-supervision scheme that requires only annotated images for training. 
%     % \wei{what is the advantage of self-supervision training? I cannot get it from your introduction.}
%     \vspace{-0.08cm}
%     \item Experiments on COCO-stuff~\cite{cocostuff} dataset that show significant improvements over existing methods. Moreover, our model provides interpretability and can be extended to other tasks of content manipulation.
% \end{itemize}

% % In this paper, we proposed a learning-based approach that learns style consistency from data. Our assumption is that if two patches come from the same image, their styles are consistent. Using style-consistent patches cropped from the same image, the discriminator implicitly learns the style-consistent constraint.
% % Using paired tuples $(x,c)$, a discriminator can learn the style consistency constraint by predicting if a new $x,c$ is real.
% % However, since every two images have different styles, it is hard to collect $(x,x_ref)$ tuples. To solve this problem, we proposed a self-supervised approach. We assume two patches from the same image share the same style. By cropping non-overlapping patches from a large image, $(x,x_ref)$ patch tuples are generated, and discriminator can learn style consistency using the generated tuples. \TDOD{add previous works
% %https://github.com/jason718/awesome-self-supervised-learning#image-representation-learning
% % }


% % From the generator perspective, another challenge is that reference image $x_s$ contain multiple regions, and is not aligned to the output. Therefore, standard convolutional generators~\cite{dcgan,pix2pix} cannot effectively propogate style information from the reference image. To overcome this limitation, Xun \etal~\cite{munit} apply global average pooling to encode style information. However, visual features may be corrupted if features from multiple regions are averaged. Differently, Wang \etal~\cite{vid2vid} utilize optical flow for cross-frame alignment. 

% % Another challenge designing a network structure which is suitable for constrained prediction. The existing network 

% % Challanges 1: first, how to define the style constriat? for strutural constrain, there are paired data as supervision. Using the paired GT, the discriminator learn to judge if two paris are aligned. However, there no supervision for our task, i.e. no paired data (hard to collect data) which has exact same style.  Previous work: ??? (check self supervision paper
% %https://github.com/jason718/awesome-self-supervised-learning#image-representation-learning
% % ) . Solution: patch-based self-supervision

% % Challanges 2: even we get paried data, by default the convolutional network (U-Net) is good at strucutral prediciton. But, because since the reference image has arbitary content, the output image is un-aligned to reference image. We need to design an alignment module. Previous work: flow: not good, self-attention: not good. high complexity, double attention.  Solution: a two stage attentnion

% % Challanges 3: handle occlusion and new semantic regions.
% % Solution 3: masking global features.


% % Because the reference image can be of random structure (different from the conditional input), alignment becomes crucial. To tackle this challenge, we present an global-local attention mechanism to transfer information form the reference image. To properly generate missing content, we uses global filtering to un-attend features when doing inference. Finally, we proposed a novel patch-based data scheme with systematical designed disentangled encoder-decoder to enable the training our model.


% % \section{Introduction}
% % The key to our approach: we assume patches in the same image share the same style coding $s$. However images with the same style can have vastly different content $c$ (show figure), therefore some style can be missing or in different position for each image. To model that, we use a patch coding $z$ 

% % The VAE uses graphical model $z \to x$ to model the individual patches independently. 

% % The disentangled representation separately encode learn style and content, however, it does not utilize the fact that patches in the same image has the same style. In addition, most works \cite{lee2018diverse} use concatenation to integrate style and content information.

% % In this paper, we propose a framework for reference-based image synthesis. We assume the style of the global image to be $s$. For a patch with its given content $c$, we assume a distribute function $$z = \Distribute(s|c)$$ that extract the style of a patch. A inverse processing is used $$s = \Gather(z|c)$$ to extract global style form local a patch. Using this, we are able to perform both patch encoding-decoding, and learn to transfer style. The learned \emph{Gather} and \emph{Distribute} also provide use a interpretable model that can visualize what ``style'' represent and how the reference image is transferred.


==> sections/method.tex <==

\section{Methodology}
%\subsection{Overview}
Given an image, an edited semantic layout, and a mask of the region to be modified, our task is to synthesize new image content inside the masked region such that the final completed image is visually plausible and consistent with the edited layout. Existing approaches either apply warping~\cite{cocosnet,msca} or inpainting to generate coherent contents~\cite{sesame}.
However, they lack the merits of their complimentary counterpart, i.e.~\cite{cocosnet,msca} cannot harmonize the outputs with neighboring regions and~\cite{sesame} lacks spatial alignment and discards pixels inside the mask.

To combine the advantage of both models, we propose a unified generator framework that follows the pipeline of alignment and refinement. Specifically, the alignment stage serves to generate an initial warping that is aligned to the target layout. Next, a refinement network that consists of an encoder and coarse-to-fine decoders serves to refine and harmonize the warped output. Fig.~\ref{fig:pipeline} shows an overview of our manipulation framework. We propose the high-resolution sparse attention (HRS-Att) module to efficiently and accurately transfer high-resolution visual details from the input image to the target label map by attention-based warping. We then propose a two-stage semantic layout manipulation network to generate the final manipulated output by inpainting the masked region with the guidance of the warped output. %In the following, we introduce the components of our proposed framework in detail.
%In Sec.~\ref{sec:HR_attention}, we describe HRS-Att for high-resolution warping. In Sec.~\ref{sec:network}, we describe the semantic manipulation network and its training objectives.
% In Sec.~\ref{sec:decode}, we propose a two stage decoder for edited image synthesis. Finally, in Sec.~\ref{sec:train}, we describe the training scheme of our model. 

% . As shown in Fig.~\ref{fig:generator}, our generator consists of three components, namely i) a patchmatch attention module (PMAtt) for high-resolution warping ii) an image encoding module and iii) a two-stage decoding module.
% In Sec.~\ref{subsect:HR_attention}, we propose HRAtt for high-resolution warping . In Sec.~\ref{sec:encode}, we propose an encoder for image feature encoding. In Sec.~\ref{sec:decode}, we propose a two stage decoder for edited image synthesis. Finally, in Sec.~\ref{sec:train}, we describe the training scheme of our model. 

% To this purpose, we propose an Generative Adversarial Network. As shown in Fig.~\ref{fig:generator}, our generator consists of three components, namely i) a patchmatch attention module (PMAtt) for high-resolution warping ii) an image encoding module and iii) a two-stage decoding module. In Sec.~\ref{sec:HR-attention}, we propose HRAtt for high-resolution warping . In Sec.~\ref{sec:encode}, we propose an encoder for image feature encoding. In Sec.~\ref{sec:decode}, we propose a two stage decoder for edited image synthesis. Finally, in Sec.~\ref{sec:train}, we describe the training scheme of our model. 
\vspace{-0.05in}
\subsection{Cross-domain Correspondence}
Computing a dense correspondence between the image and the edited layout is a crucial first step for local layout editing, as we need to warp input visual details to fit the target layout while making the warped image visually plausible.
%Our problem is to transfer visual details from an image $x \in \mathbb{R}^{H \times W \times 3}$  to its edited semantic layout $c \in \mathbb{R}^{H \times W \times C}$  consisting of $C$ semantic classes.
Recently, Zhang et.~al~\cite{cocosnet} propose a cross-domain correspondence network for layout-guided alignment.
% Specifically, it first transforms the input image $x \in \mathbb{R}^{H \times W \times 3}$ and the edited label map $c \in \mathbb{R}^{H \times W \times C}$ (consisting of $C$ semantic classes) to a shared domain with
\zht{Specifically, it first transforms the input image $x \in \mathbb{R}^{H \times W \times 3}$ and the edited label map $c \in \mathbb{R}^{H \times W \times C}$ (consisting of $C$ semantic classes) to downsampled feature maps that are in a shared domain at resolution
$H/4 \times W/4$:}
%%\hz{replaced $W^\prime$ with $W/4$} 
% $H^\prime \times W^\prime$ ($H^\prime=H/4$ and $W^\prime=W/4$) spatial resolution using two feature extractors $F^\prime_x(\cdot)$ and $F^\prime_c(\cdot)$:
\vspace{-0.05in}
\begin{align}
\label{eq:feature_extraction}
\begin{aligned}
    f_x = F_x(x) \quad\text{and}\quad  f_c = F_c(c),
\end{aligned}
\end{align}
% \vspace{-0.05in}
% using two feature extractors $F^\prime_x(\cdot)$ and $F^\prime_c(\cdot)$:
where $F_x$ and $F_c$ denotes the cross-domain feature extractor. Here, the output features $f_x,f_c$ are normalized at each location to have zero mean and unit $\ell_2$ norm.
% simple version
% Specifically, it transforms the input image $x$ and the edited label map $c$ to a shared domain using two feature extractors: $f_x &= F_x(x;\theta_{F,x})$ and $f_c &= F_c(x;\theta_{F,c})$, where $\theta$ denotes the learnable parameters.
% \cl{what do you mean by "query location"?}
% from the dense index set $q \in \mathcal{G} = \Set{(i,j)}{0\leq i < H^\prime, 0\leq j < W^\prime}$,
% on the downsampled 2-d grid,
% $p \in \mathcal{G} = \{(i,j)|0\leq i \l H, 0\leq j \l W \}$,
Then, a low-resolution warped image $r^L \in \mathbb{R}^{{H/4 \times W/4 \times 3}}$ is calculated from the downsampled input $x^L \in \mathbb{R}^{{H/4 \times W/4 \times 3}}$ where each pixel $r^L(q)$ is computed as weighted sum of all pixels from $x^L$ \footnote{We use superscript $L$ here to denote low-resolution variables.}.
% $x^\prime \in \mathbb{R}^{H^\prime \times W^\prime\times 3}$: 
%\cl{You might not want to use $\mathcal{G}$ to refer to both feature map grid and pixels in downsampled image, right? Use two different notations?} \hz{I change grid to "2-d dense index set"}
%input pixels $q \in \mathcal{G}$ in the all spatial locations are weighted summed  to compute a warped image $r$:
\begin{align}
\label{eq:warping_dense}
\begin{aligned}
    \displaystyle
    r^L(q) &= \sum_{p} {a}^L_{q p} x^L(p),
    % {a}^L_{q p} &= {\gamma e^{s^L_{q p}}}/{\sum\limits_{p} {\gamma e^{s^L_{q p}}}}
\end{aligned}
\end{align}
where $p$ iterates over all spatial locations of $x^L$, ${a}^L_{q p} = {\gamma e^{s^L_{q p}}}/{\sum_{p} {\gamma e^{s^L_{q p}}}}$ is the linear weight computed from the inner-product feature similarity $s^L_{q p}=\langle f_c(q),f_x(p) \rangle$ and $\gamma$ is a temperature coefficient.
% Here, $f_c(q)$ and $f_x(p)$ are normalized to have
% \zl{is "s" computed as cosine similarity? are features normalized?}
% \todo{normalize feature, put gamma in softmax, add footnoot superscript L, put a in text.}

% \cl{I don't understand the following sentence. What do you mean "mapped to an output"?}
%\cl{The following paragraph is still confusing. What is $f_c$. why ``pixels (p)", cannot we just say ``pixels"? }\hz{revised}
%\cl{I still don't understand the following sentence honestly. is the $q$ in the sentence below the same q as in line 342 $q \in \mathcal{G}$? It sounds like q here refers to a different thing in which case using q in both places is confusing.} \hz{I revised the text so that all $q$ and $p$ comes from Eq (2). Not sure if its the best way to introduce query key.}
The warping function of Eq.~\ref{eq:warping_dense} can be interpreted as an attention operation~\cite{vaswani2017attention}, 
where each index $q$ (query) is mapped to a weighted sum of pixels (value) of index $p$ (key). 
%In this paper, we adopt the terminology query and key to refer to $q$ and $p$, respectively.
%\cl{You might want to explicitly call out what $v$ ,$p$ and $q$ in the attention metaphor are in our case? $v$ is probably the $p$ defined earlier (pixel values from downsampled image $x^\prime$? what is the key ($p$) in our case?}\hz{revised}
% The warping operation defined by Eq.~\ref{eq:warping_dense} 
However, such a mapping step needs to compute pair-wise similarity for every query and key, resulting in a quadratic computation complexity w.r.t. the spatial resolution.
% As the complexity grows quadratically with respect to the spatial resolution,
Therefore, attention-based correspondence~\cite{cocosnet}
% \footnote{Recent image generation approaches including \cite{cocosnet,biggan} only explore attention module training at resolution up to $64\times64$.}
often struggles to transfer high-resolution visual details from the input image as shown in Fig~\ref{fig:teaser2}.
Note that the detailed texture in the mountains is lost in the result of CoCosNet.

\begin{figure}[t]
	\centering
	\includegraphics[width=1.\linewidth]{sections/figures/New_warping.jpg}
	\caption{
% 	Our HRS-Att utilizes the proposed key index sampling step to generate sparse indexes and then apply?  sparse attention warping to perform attention-based summation on an irregular grid.
	Our HRS-Att utilizes key index sampling step to generate sparse key indexes for sparse attention computation.
% 	\zl{try to use ligher colors for fc, fx background color.} \hz{done}
	}
	\label{fig:sparse_attention}
\end{figure}



\subsection{High-resolution Sparse Attention}
\label{sec:HR_attention}
\zht{
Image correspondence is often sparse~\cite{lowe1999object,lucas1981iterative}, meaning that for an image pair $A,B$, a pixel $A$ often matches only with a sparse set of pixels from $B$. However, the vanilla attention is inherently dense and inefficient as it looks up all pixels from $B$ to find a best match for a single pixel in $A$.
% This prevents the vanilla attention to estimate correspondence at high-resolution 
% However, the inherent dense computation of attention prevents it from computing high resolution correspondence.
% In Fig~\ref{}, we visualize a well-trained attention model~\cite{cocosnet} and find its correspondence is sparse, meaning that only a small proportion of non-zero key-value pairs contribute to the warping step.
% Actually, in Fig~\ref{}, we find that correspondence generated by a well-trained attention model~\cite{cocosnet} is sparse, meaning that only a small proportion of non-zero key-value pairs contribute to the warping step.
To make attention-based correspondence estimation feasible at higher-resolution, we propose an efficient sparse attention module. As shown in Fig~\ref{fig:sparse_attention}, our attention module consists of feature map upsampling, key index sampling and sparse attentive warping to transfer visual content up to $512\times512$ resolution.
}

% \noindent \textbf{High-resolution Cross-domain Feature Extraction.} \quad
\noindent \textbf{Feature Map Upsampling.} \quad
% \zht{To capture rich spatial details for transfer, we aim to generate high-resolution feature maps $g_x$ and $g_c$ from input image $x$ and the edited label map $c$, respectively, at resolution $H\times W$.}
% Given the input image $x$ and the edited label map $c$, we aim to generate high-resolution feature maps $f_x, f_c$ at resolution $H\times W$ to capture rich spatial details for transfer.
\zht{To capture rich spatial details for transfer, we generate high-resolution cross-domain feature maps $u_x$ and $u_c$ from the low-resolution inputs $f_x$ and $f_c$. In particular, we apply spatially adaptive normalization~\cite{spade} to sequentially upsample the input feature until resolution $H\times W$:}
\begin{align}
\label{eq:feature_upsample}
\begin{aligned}
    u_x = U_x(f_x, c) \quad\text{and}\quad  u_c = U_c(f_c, x),
\end{aligned}
\end{align}
% \todo{explain Gx, Gc, use Ux, Uc}
where $U_x(f_x;c)$ and $U_c(f_c, x)$ are two SPADE~\cite{spade} feature upsamplers that take $c$ or $x$ as guidance to upsample $f_x$ or $f_c$. We perform channel-wise normalization at the end of $U_x$ and $U_c$, such that the output features at every locations are normalized to have zero mean and unit $l_2$ norm.

\begin{figure}[]
	\centering
	\includegraphics[width=.9\linewidth]{sections/figures/correspondence.png}
	\caption{The warping and synthesis results of our method against CoCosNet~\cite{cocosnet}. Our HRS-Att can transfer high-resolution details for better semantic layout manipulation.}
	\label{fig:teaser2}
\end{figure}

\noindent \textbf{Sparse Attention.} \quad
% \cl{Why is this a fact? Is there a reference to cite or something?}
Motivated by the sparsity of correspondences, 
%we propose to prune the search space of keys in the attention step. Specifically, 
for each query $q$, we constrain the search space of keys $p$ to be in a sparse key set $\mathbb{K}_q$ where $|\mathbb{K}_q|\ll H W$. Therefore, Eq.~\ref{eq:warping_dense} becomes: 
%a high-resolution and sparsified version:
\vspace{-0.05in}
\begin{align}
\label{eq:warping_sparse}
\begin{aligned}
    \displaystyle
    r(q) &= \sum_{p \in \mathbb{K}_q} a_{q p} x(p),
    % {a}_{q p} &= {e^{s_{q p}}}/{\sum\limits_{p \in \mathbb{K}_q} {e^{s_{q p}}}},
\end{aligned}
\end{align}
% \vspace{-0.05in}
\zht{where $p$ iterates over the sparse key set $\mathbb{K}_q$, ${a}_{q p} = {\gamma e^{s_{q p}}}/{\sum_{p \in \mathbb{K}_q} {\gamma e^{s_{q p}}}}$ is the normalized weight computed from $s_{q p}=\gamma \langle u_c(q),u_x(p) \rangle$, the high-resolution feature similarities. Next}, we propose a key index set sampling step to generate $\mathbb{K}_q$ and a sparse attentive warping module that efficiently aggregates pixels over $\mathbb{K}_q$.
%  \cl{What do you mean by irregular grid?}
% \todo{$\mathbb{K}_q$ change to $\mathbb{K}_q$}
% \todo{normalize feature, put gamma in softmax, add footnoot superscript L, put a in text.}

\noindent \textbf{Key Index Sampling.} \quad
% \zht{To efficiently generate the sparse key set $\mathbb{K}_q$, we leverage the  }
Motivated by a randomized correspondence algorithm, PatchMatch~\cite{patchmatch}, we propose the key index sampling step to exploit the spatial coherency of feature correspondences for efficient index set generation.
%\zht{Different from PatchMatch, our goal is to generate multiple samples for each query to enable sparse attention rather than computing the best match. Moreover, we leverage tensor operation~\cite{duggal2019deeppruner} to make the key index sampling compatible with the learning-based correspondence pipeline. Finally, as described later, we made several testing stage customization to improve local editing.}
% \hz{
% patchmatch is efficient algorithm to find correspondenc, but not good for our case. we are not interested in  interested in finding key index set to . We dev for sparse attention
% - dynimic generate multiple sample sample as key set
% - for correspondence pipeline, tensor operation \cite{supp_duggal2019deeppruner} using convolution.
% - testing time for  customize for local edit describe later.
% }
% \zl{what's the difference and advantage of KIS from/over PM. Why we come up a new method rather than use PM directly? We need to list all the differences and maybe highlight some of them to differentiate ours from PM} \hz{revised}
Specifically, for each query position $q$, we append a randomly initialized particle $\mathbf{t}_q=(t_q^x, t_q^y)$ to the index set $\mathbb{K}_q$ as initialization, namely $\mathbb{K}_q=\{\mathbf{t}_q\}$. Moreover, we use notation $\mathbb{P}_q$ to denote a ``search pool'' for each location $q$.
% used for searching better matched particles.
To ensure that $\mathbb{K}_q$ covers the best matches, we alternate between a \textit{initialize-propagate-evaluate} step that updates $\mathbf{t}_q$ with a better matched particle and an \textit{accumulation} step that appends the current particle $\mathbf{t}_q$ to $\mathbb{K}_q$:
\begin{enumerate}
    \vspace{-0.1in}
    \item Initialize: to update $\mathbf{t}_q$ with better matching, a search pool $\mathbb{P}_q$ is initialized at each location $q$ with $\mathbf{t}_q$ and $k$ random particles sampled in the neighboring space of $\mathbf{t}_q$, resulting in  $\mathbb{P}_q=\{\mathbf{t}_q\}\cup \{{\mathbf{t}_q+w\mathbf{R}^{(i)}}\}$, where $\mathbf{R}^{(i)}$ is a random vector uniformly sampled in $[-1,1]\times[-1,1]$, $w$ is a predefined window size and $0\leq i<k$;
    \vspace{-0.1in}
    \item Propagate: to leverage spatial coherency, search pool $\mathbb{P}_{q^\prime}$ from $q^\prime\in N(q)$, the adjacent pixel of $q$ are propagated to $\mathbb{P}_q$, resulting in: $\mathbb{P}_q \gets \mathbb{P}_q\cup \bigcup_{q^\prime\in N(q)} \mathbb{P}_{q^\prime}$;
        \vspace{-0.2in}
    \item Evaluate: particles from $\mathbb{P}_q$ with the maximal feature matching score is used to update $\mathbf{t}_q$, resulting in $\mathbf{t}_q \gets \argmax_{\mathbf{t} \in\mathbb{P}_q} s_{q t}$
        \vspace{-0.1in}
    \item Accumulate: the current match $\mathbf{t}_q$ is appended to $\mathbb{K}_q$: $\mathbb{K}_q \gets \mathbb{K}_q \cup \{\mathbf{t}_q\}$.
\end{enumerate}
\vspace{-0.05in}
The above procedure is repeated $N-1$ times where all the sub-steps are in parallel for each $q$. 
Fig.~\ref{fig:corr_visualize} shows that our procedure can sample diversified particles including random ones and most matched ones. 
% One would argue that the index set $\mathbb{K}_q$ should only contain those best matched particles. However, by including randomized key position, we provide richer gradients w.r.t. the feature maps for better error backpropagation. \todo{do toy experiment}
To sample even more key indices, we initialize, update and append $M$ particles $\mathbf{t}_q^{(k)} (0<k\leq M)$ in parallel following the same procedure, resulting in a total of $M N$ index samples for each query.

It is shown that the above propagation step can be implemented via convolution~\cite{duggal2019deeppruner}. The other steps can be implemented by build-in tensor operations. 
%As a result, the proposed sampling procedure is efficiently implemented using tensor operations. 
Please refer to the appendix for the pseudo code of the sampling procedure.

% Accordingly, we record the matching scores of each particles to facilitate further computation.
% The above procedure generates a set of unmatched to matched points at each evaluation iteration, which are added to the point set $\mathbb{K}_p$ at each location $p$. \cl{What do you mean by "unmatched to matched points"?}Note that the matching scores $S_{p,q}, q\in\mathbb{K}_p$ are also computed during the above procedure. 
% Details of the key index sampling step are shown in Algorithm~\ref{algorithm:sampling}. 
% Similar to~\cite{duggal2019deeppruner}, we convolve particle indices with predefined kernels to implement 
% the particle propagation step. Moreover, the evaluation step is implemented with build-in array indexing operation and feature matching. Please refer to the appendix for details of Algorithm~\ref{algorithm:sampling}.
% Note that the key index sampling algorithm can be efficiently implemented using standard convolution operations.by unrolling the standard neural network layers. \cl{What do you mean by "unrolling"?}
% \todo{Add a figure to show the index with iteration (coordinate map and a specific result).}


% \begin{algorithm}[h]
% \DontPrintSemicolon
% \SetAlgoLined
% \SetNoFillComment
% \LinesNotNumbered 
% %\SetSideCommentLeft
%  \KwData{$f_x^h$ and $f_c^h$: the $H\times W\times C$ feature map}
%  \KwData{N: the number of iterations}
%  \KwData{M: the number of particles}
% %   \KwData{}
% %   \begin{itemize}
% %       \item $f_x^h$ and $f_c^h$: the $H\times W\times C$ feature map
% %       \item N: the number of iterations
% %       \item M: the number of particles
% %   \end{itemize}
%  \KwResult{$\mathbf{C}$: the $NM\times H\times W\times 2$ key index sets}
% %  \KwResult{$\mathbf{S}$: the $NM\times H\times W$ feature matching scores}
%  \tcc{Randomly initialize $M$ particles $\mathbf{t}$ of size $M\times H\times W\times 2$}
%  $\mathbf{C} \gets \emptyset$;
%  $\mathbf{t}_{x} \sim U(0,W)$; $\mathbf{t}_{y} \sim U(0,H)$\;
%  \tcc{store to outputs}
% $\mathbf{C} \gets$ insert($\mathbf{C}$, $\mathbf{z}$)\;
% %  $\mathbf{C} \gets$ insert($\mathbf{C}$, $\mathbf{q}$) \tcp*{insert particles to key index set}
%  \For{i=1...N-1}{
%     % \tcc{Particle sampling}
%     % $\mathbf{q}_{x} \sim U(0,W)$; $\mathbf{q}_{y} \sim U(0,H)$\;
    
%     \tcc{Propagation by convolution}
%     $\mathbf{t} \gets \mathbf{t} \circledast \mathbf{k_h}$ \tcp*{horizontal propagation}$\mathbf{t} \gets \mathbf{t} \circledast \mathbf{k_v}$ \tcp*{vertical propagation}
%     % \tcc{Evaluation by top-M match selection}
%     % \tcc{Evaluation}
%     \tcc{Evaluate top-M match}
%     $\mathbf{t} \gets $evaluation($\mathbf{q}, f_x^h, f_c^h,M$)\;
%     % $\mathbf{q} \gets $evaluation($\mathbf{q}, f_x^h, f_c^h,M$)\tcp*{top-M match selection}
%     \tcc{store to outputs}
%     $\mathbf{C} \gets$ insert($\mathbf{C}$, $\mathbf{t}$)\;
%     \tcc{Particle Sampling}
%     % $\mathbf{q}_{x} \sim U(0,W)$; $\mathbf{q}_{y} \sim U(0,H)$\;
%     $\Delta \mathbf{t}_{x} \sim U(0,W)$; $\Delta \mathbf{t}_{y} \sim U(0,H)$\;
%     $\mathbf{t}_{x} \gets$ insert($\mathbf{t}_{x}, \Delta \mathbf{t}_{x}$); $\mathbf{t}_{y} \gets$ insert($\mathbf{t}_{y}, \Delta \mathbf{t}_{y}$) \;

%  }
%  \caption{Key Index Sampling.}
%  \label{algorithm:sampling}
% \end{algorithm}
% }

\noindent \textbf{Sparse Attentive Warping.} \quad
The warping operation of Eq.~\ref{eq:warping_sparse} is defined on sparse and irregular grid $\mathbb{K}_q$. 
To enable efficient implementation, we propose the sparse attentive warping operation that transforms Eq.~\ref{eq:warping_sparse} to its equivalent form via deformable convolution~\cite{deformableConv}:
\vspace{-0.1in}
\begin{align}
\label{eq:deformable}
\begin{aligned}
    \displaystyle
    r_{x\rightarrow c}(q) &= \sum_{p \in \mathbb{K}_q} a_{q p} x(p) = \sum_{k=1}^{|\mathbb{K}_q|} x(q+\Delta{q_k}) A_{qk},
    \vspace{-0.2in}
\end{aligned}
\end{align}
where $p$ enumerate all elements from $\mathbb{K}_q$, while $\Delta{q_k}=p_k-q$ and $A_{qk}=a_{q p_k}$ are the offset and modulation factor of the deformable convolution kernel defined in~\cite{deformableConv}, respectively. Note that the deformable kernel weights in Eq.~\ref{eq:deformable} are set to $1$ and thus being omitted. %\cl{If $w_k$ is always 1, why not just remove it?} \hz{$w_k$ is the kernel weight of the deformable conv}\cl{Then perhaps modify the main text to not say $w_k=1$?}
% Specifically, the matching score $s_{q,t}$ for $t \in \mathbb{K}_q$ is normalized via softmax. Next, the sparse attention-based warping is efficiently implemented using the a variant of deformable convolution~\cite{deformableConv}. Formally, 
% \begin{align}
% \label{eq:warping_sparse}
% \begin{aligned}
%     \displaystyle
%     r_{x\rightarrow c}(q) &= \sum_{p \in \mathbb{K}_q} a_{q,p} x(p);\\
%     {a}_{q,p} &= {e^{\gamma s_{q,p}}}/{\sum\limits_{p \in \mathbb{K}_q} {e^{\gamma s_{q,p}}}},\\
% \end{aligned}
% \end{align}
% For more details of the implementation please refer to appendix.
%\cl{I know there is not enough space to talk about all details about this step. But the current paragraph does not provide enough information about what this step is making the paper not self-contained. } \hz{changed to Eq~\ref{eq:deformable}}

\noindent \textbf{Training Scheme.} \quad
% \zl{it is not very clear what we are training here, need a little more detail.} \hz{revised}
% \zht{Although the key index sampling is a non-differentiable operation that serves to prune the operation space of attention, the warped output $r$ in Eq.~\ref{eq:warping_sparse} is differentiable w.r.t. feature maps $f_x$ and $f_c$. Thus, gradients can propagate through the our sparse attention module for end-to-end training.}
\zht{
We follow the training scheme of~\cite{cocosnet} to train our sparse attention module. Specifically, after attention-based warping, the warped image is fed to a SPADE~\cite{spade} generator to synthesize the layout-transferred image. The loss defined on generated image and other losses will be backpropagated to jointly update feature extractors of the sparse attention module and the generator. Although the key index sampling procedure is non-differentiable, the warped output $r$ in Eq.~\ref{eq:warping_sparse} is differentiable w.r.t. feature maps $f_x$ and $f_c$. Gradients can thus propagate through the sparse attention module for training.}

% \zht{
% We follow the data scheme and training objectives of~\cite{cocosnet} to learn the sparse attention module. Specifically, warped images $r_{x\rightarrow c}$ are fed to a SPADE generator~\cite{spade} such that outputs $\hat{y}_{x\rightarrow c}$ follows the style of $x$ and the layout of $c$. To generate paired data for training,  image-layout pairs $(x_0,c_0)$ from the ADE20k dataset is spatially augmented to new image-layout pairs $(x_1, c_1)$ via random translation and flipping. Next, images with similar semantic to $x_0$ and its label map, denoted by $(x_2, c_2)$, is retrieved as unpaired data.

% Following~\cite{cocosnet}, our training objective consists of domain alignment loss $\mathcal{L}_{\text{domain}}=\norm{f_{x_0}-f_{c_0}}_1$, feature matching loss $\mathcal{L}_{\text{feat}}=\sum_l{\lambda_l \norm{\phi_l(\hat{y}_{x_1\rightarrow c_0})-\phi_l(x_0)}_1 }$, perceptual loss~\cite{perceptual} $\mathcal{L}_{\text{perc}}=\norm{\phi_l(\hat{y}_{x_2\rightarrow c_0})-\phi_l(x_2)}_1$ and contextual loss~\cite{contextual} $\mathcal{L}_{perc}=\contextual(\hat{y}_{x_2 \rightarrow c_0}, x_2)$.
% To stabilize training, we also impose constraints on the downsampled feature maps. Specifically, let $f_x^l, f_c^l$ denote the downsampled version of $f_x, f_c$ at resolution $H^\prime \times W^\prime$. 
% We enforce the constraint that the input image should be cycle-consistent to the forward-backward warped image in low-resolution:
% \begin{align}
% \label{eq:loss_align_cycle}
% \begin{aligned}
%     \mathcal{L}_{cycle} = \norm{r^l-r^l_{cycle}},
% \end{aligned}
% \end{align}
% where $r^l(q) = \sum_{p\in \mathcal{G}^\prime} \softmax (\gamma s^l_{q,:})_p x^\prime(p)$ and $r^l_{\text{cycle}}(q) = \sum_{p\in \mathcal{G}^\prime} \softmax(\gamma s^l_{:,q})_p r^l(p)$ are the forward and forward-backward warped images in low-resolution, respectively, $s^l_{q,p}=\langle f_c^l(q), f_x^l(p) \rangle$ denotes the matching score on the downsampled feature maps, $s^l_{q,:}$ and $s^l_{:,q}$ select the q'th row and column from matrix $(s^l_{i,j})_{ij}$, respectively.}

\zht{
We denote the synthesized output that follows the style of $x$ and the layout of $c$ as $y_{x\rightarrow c}$.
Following~\cite{cocosnet}, data pairs $(x_0,c_0)$ is sampled from the ADE20k dataset. Then, a new pair $(x_1, c_1)$ is spatially augmented from $(x_0,c_0)$ and $y_{x_1\rightarrow c_0}$ is synthesized by the model. Moreover, images with similar semantic to $x_0$ and its label map, denoted by $(x_2, c_2)$, is retrieved and $y_{x_2\rightarrow c_0}$ is synthesized.
Similar to~\cite{cocosnet}, our training objective consists of domain alignment loss, feature matching loss, perceptual loss~\cite{perceptual} and contextual loss~\cite{contextual}.
To stabilize training, we also impose regularization on the downsampled feature maps which is provided in the Appendix.
% Specifically, let $u_x^L, u_c^L$ denote the downsampled version of $u_x, u_c$ at resolution $H/4 \times W/4$. 
% We constrain that the input image should be cycle-consistent to the forward-backward warped image in low-resolution:
% \vspace{-0.1in}
% \begin{align}
% % \label{eq:loss_align_cycle}
% \begin{aligned}
%     \mathcal{L}_{cycle} = \norm{r^L_u-r^L_{cycle}},
%     % \vspace{-0.05in}
% \end{aligned}
% \end{align}
% where $r^L_u(q) = \sum_{p} \softmax (\gamma t^L_{q:})_p x^L(p)$ and $r^L_{\text{cycle}}(q) = \sum_{p} \softmax(\gamma t^L_{u,:q})_p r^L_u(p)$ are the forward and forward-backward warped images in low-resolution, respectively, $s^L_{q,p}=\langle u_c^L(q), u_x^L(p) \rangle$ denotes the matching score on the downsampled feature maps, $t^L_{q:}$ and $t^L_{:q}$ select the q'th row and column from matrix $(t^L_{ij})_{ij}$, respectively.
}
% \cl{what is $\mathcal{G}^\prime$}
% \todo{remove G, say low resolution}



%\cl{what are $s^l_{q,:}$ and $s^l_{:,q}$?}
% In addition, we impose a KL-divergence loss on  such that the low-resolution correspondence is similar to the high-resolution correspondence of $\softmax\limits_{q \in \mathcal{G}^l}$ 
% \todo{attention non-differnable, feature is differentalbe?}\\
% \todo{training detail, why backpropagate train feature.\\ Important. Patchmatch non-differanble challange}\\ 
% \todo{add a training detail section, explain why patchmatch can not differentiable but can be used to update feature map. Also mention some papers on randomized sparse attention.}
% \todo{Also mention some papers on randomized sparse attention.}

\noindent \textbf{\zht{Customization for Local Editing.}} \quad
% \zl{Need to motivate a bit on our main task is "local manipulation and directly apply global warping does not work for local editing.."}
Our sparse attention module is trained and applicable to the global alignment task of~\cite{cocosnet}.
\zht{However, the global correspondence does not take the contextual constraint into account for the task of local layout manipulation, causing inconsistency at boundary of editing region. Moreover, misalignment can be further reduced by encouraging correspondence smoothness and adopting the following customization to the key index sampling step:}
i) to avoid semantic mismatching, in the inference step, we add a large penalization constant to $s_{q t}$ if $q$ and $t$ belong to different semantic regions, ii) in the sampling step, we exponentially decay the window size $w$ as the iteration number increases, and iii) we repeat more propagate-evaluation steps in each iteration to enforce correspondence smoothness. The optimized procedure helps to improve the warping quality for local editing.
% \zl{I would add more details or even figure for this section, which is more novel.} \hz{revised}

\subsection{Semantic Layout Manipulation Network}
\label{sec:network}
As shown in Fig.~\ref{fig:pipeline}, our semantic layout manipulation network takes an image $x_0$, an edited layout $c_1$ and a mask $m$ which indicates the region to-be-edited as inputs. Our generator denoted by $G$ aims to hallucinate new pixels inside the mask to generate the edited image $y$:
\begin{align}
\label{eq:generator}
\begin{aligned}
    y = G(x_0,c_1,m) \odot m + x_0 \odot (1-m),
\end{aligned}
\end{align}
whereas the generated contents inside the mask should be i) aligned to the layout $c_1$ and ii) coherent with the neighboring content $x_0 \odot (1-m)$. 

\noindent \textbf{High-resolution Local Alignment.} \quad
Aiming at transferring visual details from the input image to handle drastic layout change, we first apply spatial alignment described in Sec.~\ref{sec:HR_attention} to generate an layout-aligned image $r_{x_0\rightarrow c_1}$ that is consistent to $x_0$ and follow the layout of $c_1$. The pixels outside the mask are then replaced by the real image, resulting in a \textit{locally warped} image:
% \cl{I don't understand the previous sentence. Is there a mistake in the equation below?}
\begin{align}
\label{eq:local_align}
\begin{aligned}
    x_{\text{warp}} = r_{x_0\rightarrow c_1} \odot m + x_0 \odot (1-m).
\end{aligned}
\end{align}
As the locally warped images $x_{\text{warp}}$ may contain appearance discontinuity due to misalignment, we next propose a generator that consists of a semantic encoder and coarse-to-fine decoders to refine the warped result.

\noindent \textbf{Semantic Encoder.} \quad
To better capture semantic and structure clue from the noisy output $x_{warp}$, we use a pretrained visual-semantic embedding (VSE) model~\cite{vse++} to extract multi-scale visual features $f^{(1)}, f^{(2)}, f^{(3)}, f^{(4)}  = \VSE(x_\text{warp})$.
% \begin{align}
% \label{eq:encode}
% \begin{aligned}
%     f^{(1)}, f^{(2)}, f^{(3)}, f^{(4)}  = \VSE(x_\text{warp}).
% \end{aligned}
% \end{align}
Likewise, we extract layout embedding $f_{c_1}$ from the one-hot layout label map of $c_1$ using a $1\times 1$ convolution layer.


\zht{
\noindent \textbf{Coarse-to-fine Synthesis} \quad
As the warping result $x_\text{warp}$ may contain misalignment artifact as shown in Fig~\ref{fig:pipeline}, we propose a coarse-to-fine refinement network to refine $x_\text{warp}$. 
In particular, our coarse-stage network consists of a two-branch encoder that utilizes dilated convolution~\cite{dilatedconv} and contextual attention~\cite{deepfillv1} to propagate visual information from the neighboring regions of $x_0$. The two-branch encoder takes the concatenation $[x_\text{warp},f_{c_1},m,x_0\odot (1-m)]$ as input to extract multi-scale features. Furthermore, at each scale $i$ of the two-branch encoder, visual features at the same scale $f^{(i)}$ and the resized layout embedding $f_{c_1}$ are also concatenated to help propagating contextual information. After concatenating the two feature maps generated by the encoders, a coarse stage decoder that consists of multiple deconvolution layers sequentially upsample feature resolution and produce an coarse image prediction $y_{\text{coarse}}$.
%\cl{What do you mean "highest scale"?} \hz{done}

% Based on the first-stage network, we 
% As shown in Fig~\ref{fig:pipeline}, our first-stage network utilizes dilated convolution~\cite{dilatedconv} and contextual attention~\cite{deepfillv1}
% to aggregate information from the real neighborhood and to make an initial coarse prediction.
% In particular, the first-stage network takes layout $c$, mask $m$ and the warp image $x_{warp}$ as inputs. Moreover, semantic encoder features  $f^{(i)}$ are consecutively concatenated to the encoder of the first-stage model to inject more high-level information.

Motivated by the coarse-to-fine pipeline~\cite{deepfillv1,xiong2019foreground} of inpainting models, we employ a refinement network based on SPADE~\cite{spade} to refine $y_{\text{coarse}}$. However, we feed the intermediate features from the coarse-stage decoder $f_{\text{if}}$ and $[x_\text{warp},y_{\text{coarse}},f_{c_1},m]$ as additional inputs to our refinement network, such that the contextual information from the coarse-stage network and inputs can be exploited.
}

\zht{
\noindent \textbf{Self-supervised Training} \quad
It is hard to collect ground-truth triplets $(x_0,c_1,x_1)$ such that the edited groundtruth $x_1$ is aligned to the layout of $c_1$ while being coherent with neighboring content of $x_0$. However, assuming such $x_1$ exists, $x_0$ will only be involved in Eq.~\ref{eq:local_align} in our network to generate the warped image $r_{x_0\rightarrow c_1}$.\footnote{Whereas the neighboring content of the input image $x_0 \odot (1-m)$ can be the neighboring content of  $x_1$, namely $x_1 \odot (1-m)$.} This motivate us to  design a novel unsupervised scheme that relies on approximated warped content $r_{x_0\rightarrow c_1}$ instead of $x_0$ to generate the edited output.

Specifically, during training, we sample image-layout pairs $(x_1, c_1)$ from datasets and free-form mask $m$ using the procedure described in~\cite{deepfillv2}. Instead of collecting $x_0$, we apply random translation on $x_1$, resulting in augmented image $\widetilde{x}_1$. Since $x_0,x_1$ and $\widetilde{x}_1$ are coherent in content, we approximate $r_{x_0\rightarrow c_1}$ with $r_{\widetilde{x}_1\rightarrow c_1}$ whereas the locally warped image in Eq.~\ref{eq:local_align} is replaced by:
%\cl{It is not clear what is $x_2$. Also why is it $r_{x_2^\prime\rightarrow c_1}$ but not $r_{x_2\rightarrow c_1}$ in the equation?} \hz{done}
\begin{align}
\label{eq:local_align2}
\begin{aligned}
    x_{\text{warp}} = r_{\widetilde{x}_1\rightarrow c_1} \odot m + x_1 \odot (1-m).
\end{aligned}
\end{align}

We first train the first-stage network using a combination of pixel-wise $\ell_1$ loss and perceptual loss~\cite{perceptual} to give coarse prediction. 
% \cl{Why is there both a ``training details" here and a "4.1 implementation details" later?}
% \begin{align}
% \label{eq:xx}
% \begin{aligned}
%     \mathcal{L}_{stage-I} = \norm{x_{out1}-x}_1 + 
%     \mathcal{L}_{TV}(\mathbf{w}^{(l)}_{t\rightarrow s}) =  {\norm{\frac{\partial}{\partial x}\mathbf{w}^{(l)}_{t\rightarrow s}}_1} + {\norm{ \frac{\partial}{\partial y}\mathbf{w}^{(l)}_{t\rightarrow s}}_1}.
% \end{aligned}
% \end{align}
Subsequently, the second-stage network is jointly trained with the initially trained first-stage network using a combination of two-stage pixel-wise $\ell_1$ loss, perceptual loss~\cite{perceptual} $\mathcal{L}_{\text{prec}}$ and adversarial loss to give the final output:
% \zl{coarse-to-fine network is finetuned from the initially trained first-stage network? The name "first-stage" and "coarse-to-fine" are confusing}\hz{revised}
\begin{align}
\label{eq:generator_loss}
\begin{aligned}
    \mathcal{L}_G = &\lambda_{\ell 1} \mathcal{L}_{\ell \text{1-stage1}} + 
                    \lambda_{L1} \mathcal{L}_{\ell \text{1-stage2}}+ \\ &\lambda_{\text{prec}} \mathcal{L}_{\text{prec}} - \lambda_{\text{adv}} \mathop{\mathbb{E}}_{z\sim p(z)}[D(y,c,m)],
\end{aligned}
\end{align}
where $\lambda$ represents the balancing terms. For discriminator, we apply the Markovian discrinimator~\cite{deepfillv2} with hinge loss:
\begin{align}
\label{eq:discriminator_loss}
\begin{aligned}
    \mathcal{L}_D = & \mathop{\mathbb{E}}_{z\sim p_{\text{data}}}[\sigma(1-D(x,c,m))] + \mathop{\mathbb{E}}_{z\sim p(z)}[\sigma(1+D(y,c,m))].
\end{aligned}
\end{align}
}


==> sections/related.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.8\linewidth]{sections/figures/New_pipeline.jpg}
	\caption{
	Overall pipeline of our semantic layout manipulation framework. We propose a high-resolution sparse attention module to generate the warped image with semantically aligned appearances (left). Then, a unified semantic layout generator consisting of a semantic encoding network and a coarse-to-fine decoding network is proposed to predict the final refined result.
% 	\zht{TODO: redraw the figure}
% 	\zl{redraw the figure with a new image example to make the inputs to the generator clear.}
	}
	\label{fig:pipeline}
	\vspace{-0.2in}
\end{figure*}

\vspace{-0.2in}
\section{Related Work}
\noindent \textbf{Image Synthesis and Manipulation.} \quad
Image synthesis and manipulation has a long standing history. Early works on image manipulation apply non-parametric modeling of patches~\cite{efros1999texture,image_analogies} or copy-pasting patches~\cite{patchmatch,cho2008patch} to synthesize images. Recently, with the advances of generative adversarial networks (GANs)~\cite{gan,wasserstein,lsgan,improved,sagan,largescalegan,stylegan,progressivegan}, image synthesis and manipulation tasks including style transfer \cite{cyclegan,liu2017unsupervised,munit,drit,pairedcyclegan}, photo-realistic synthesis~\cite{pix2pix,pix2pixhd,CRN,spade}, inpainting~\cite{deepfillv1,deepfillv2,structureflow,spg,edgeconnect} and editing~\cite{zhu2016generative,bau_semantic,liu2020open} has made substantial progresses.

\noindent \textbf{Layout-guided Image Manipulation.} \quad
Layout-guided image manipulation aims to modify an input image such that the generated image conforms to a desired layout.
For layout-based image manipulation, Zhu~\etal~\cite{zhu2016generative} apply optimization with layout constraints to update images.
Recently, layout guidance has been used to improve inpainting. In particular, two-stage models~\cite{xiong2019foreground,edgeconnect} are designed to generate edge maps from inputs for better result quality. Song~\etal~\cite{spg} use a pre-trained segmentation network to improve inpainting results. Although those works are  designed for inpainting, the guided synthesis framework has inspired a later work~\cite{sesame} for semantic layout manipulation. Specifically, the model of~\cite{sesame} uses local semantic label map as the guidance to manipulate masked images. 

\noindent \textbf{Example-guided Synthesis.} \quad
% Semantic Layout Manipulation is also closely related to example-guided synthesis. 
% Example guided synthesis aims to synthesize a new image such that it follows the style of an example input image. Different from image manipulation, 
Example-guided synthesis~\cite{example_cvpr19,cocosnet,msca} aims to transfer the style of an example image to a target condition, (e.g. a semantic label map).
Different from image manipulation, the generated layout can be very different from the exemplar.
% The initial work of~\cite{example_cvpr19} concatenates target condition with exemplar to generate outputs with desired styles.
To transfer visual style from the exemplar, attention-based warping schemes are proposed. Specifically, Zhang~\etal~\cite{cocosnet} propose a cross-domain attention module to transfer pixel from exemplar. Zheng~\etal~\cite{msca} propose a masked spatial-channel attention for multi-scale feature alignment. 

\noindent \textbf{Efficient Attention.} \quad
The attention mechanism~\cite{bahdanau2014neural} is shown effective for layout alignment tasks~\cite{cocosnet,msca,ren2020deep}.
However, they cannot be easily adapted to higher resolution due to the high computational cost.
Recent works focus on approximating the attention with more efficient formulation. Specifically, low-rank decomposition~\cite{doubleattention,msca}, criss-cross attention~\cite{CCA} and Taylor series expansion~\cite{GCNL} are proposed to approximate attention.
In this work, we exploit the spatial coherence of correspondences and sparse sampling to accelerate attention.

% The self-attention~\cite{wang2018non,sagan} can capture general pair-wise correspondences. However, it is computationally intensive at high-resolution. \zht{To enable fast attention computation, GCNL~\cite{GCNL} and CCCA~\cite{CCA} respectively apply Taylor series expansion and criss-cross attention to approximate self-attention. Alternatively, $A^2$-Nets~\cite{doubleattention} factorize self-attention to solve video classification tasks. Inspired by \cite{doubleattention}, we propose an attention-based module named MSCA. It is worth noting MSCA is based on cross-attention and feature masking for modeling image correspondence.}


